A Preliminary Study On Emerging Cloud Computing Security Challenges

Cloud computing is the internet based provisioning of the computing resources, software, and information on demand. Cloud Computing is referred to as one of most recent emerging paradigms of computing utilities. Since Cloud computing is the dominant infrastructure of the shared services over the internet, it is important to be aware of the security risk and the challenges associated with this emerging computing paradigm. This survey provides a brief introduction to the cloud computing, its major characteristics, and service models. It also explores cloud security threats, lists a few security solutions , and proposes a promsing research direction to deal with the evolving security challenges in Cloud computing.

==> challenges.tex <==
Responding to a true positive flag the IDS needs to then decide on how to manage the situation. Triggering a warning to the driver or by disabling the CAN bus needs serious consideration and further research before implementation. There has been success with flagging an anomaly and short circuiting the CAN bus as seen in~\cite{miller2014survey} however this obviously would not be a real world solution. Tesla Motors have developed a way to shut down the CAN bus where in the case of electronic failure while the vehicle is travelling above 5mph~\cite{HackTesla} a driver is still able to retain steering and brake control which does present a solution to this problem. This can also be a fall back response of the IDS in the case of Denial of Service (DoS) attacks which are very difficult to mitigate as seen in~\cite{koscher2010experimental}. Another thing to consider would be the possibility of determining what prevention mechanism to deploy based on priority in the arbitration field in the frame~\cite{HackTesla}. To expand on this, in the CAN bus each frame transmitted contains an arbitration field which determines the logical address alongside the priority of the message to facilitate collision avoidance. Any message detected at a certain priority level or above could be used to shut down the bus in a safe manner as seen in~\cite{HackTesla} and messages with a lower priority could signal a driver to pull over when safe.
Other challenges presented by Cheng~\cite{cheng77204time} is the consideration of metrics such as accuracy (TPR/FPR), efficiency/timeliness, scalability and power consumption. Of particular importance when applied to the CAN bus is accuracy by finding a balance between false positive rate and false negative rate. Another important consideration is the timeliness of the system as process deadline violation in a real-time system such as a vehicle could have serious consequences.
Another consideration is the challenge of positioning. Options of positioning the IDS within the network is something that can affect costs and performance of the system. The following section will cover options for positioning to provide 100\% network coverage.

\subsection{On gateway ECUs}
Gateway ECUs in the CAN bus are used as an intersection between two networks with different bandwidth and baud rate~\cite{wolfhard1997can}. This presents an ideal location for an IDS/IPS due to both interfaces receiving all traffic in the network. The ideal situation would be to have IDS systems built into every gateway node in the network as identification as to which subnet an attack is originating can be determined by the interface which detects it. However, this may have a higher cost to the system so the best gateway would then be the LIN <> CAN {\color{red}I don't follow the meaning of this symbol} gateway node protecting safety-critical systems. 

\subsection{On any bus}
Due to the broadcast nature of the network it would be possible to position the IDS anywhere for it to be able to monitor all traffic as long as frame filtering is not being used. This means that the broadcast nature can potentially be used as an advantage to security. 

\subsection{High-Speed and Low-Speed bus}
In the event of frame filtering performed by gateway nodes within the network as seen in~\cite{hoppe2008security}, another option to monitor all traffic would be to position two IDSs within both the high-speed bus and the low-speed bus, however the benefits of positioning on a gateway node would outweigh this option due to the complexity involved of running two IDSs within each network.

\subsection{Software}
One final example proposed in~\cite{miller2014survey} is implementing the IDS algorithms into software around the network providing full coverage to any attack. The downside of this is potentially losing the ability to log any data which is a core feature of any IDS for future forensics and also would also be made difficult due to the low processing power of each node. 
Finally, logging data for non-repudiation and forensic evaluation would need to be incorporated as non-volatile memory would be valuable to investigators and researchers in analysing and preventing future attacks. 

